Not All Errors Are Equal: Investigation of Speech Recognition Errors in Alzheimer's Disease Detection

Automatic Speech Recognition (ASR) plays an important role in speech-based automatic detection of Alzheimer's disease (AD). However, recognition errors could propagate downstream, potentially impacting the detection decisions. Recent studies have revealed a non-linear relationship between word error rates (WER) and AD detection performance, where ASR transcriptions with notable errors could still yield AD detection accuracy equivalent to that based on manual transcriptions. This work presents a series of analyses to explore the effect of ASR transcription errors in BERT-based AD detection systems. Our investigation reveals that not all ASR errors contribute equally to detection performance. Certain words, such as stopwords, despite constituting a large proportion of errors, are shown to play a limited role in distinguishing AD. In contrast, the keywords related to diagnosis tasks exhibit significantly greater importance relative to other words. These findings provide insights into the interplay between ASR errors and the downstream detection model.

==> figs/cookie.tex <==
\begin{figure}[htb]
\centering
\includegraphics[width=0.9\linewidth]{figs/cookie.jpg}
% \vspace{-1em}
\caption{The Cookie Theft Picture.}
\label{fig:cookie}
\end{figure}


==> tables/cases.tex <==
\begin{table*}[htbp]
\hspace{-0.25cm}
\centering
\caption{
xxx
}
\label{tab:cases}
\scalebox{0.9}{
\setlength{\tabcolsep}{4pt} % column spacing
\renewcommand{\arraystretch}{1.3} % line hight

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\begin{tabular}{l|c|c|l|}
\toprule

\textbf{id} & \textbf{Trans. } & \textbf{WER} & \textbf{Example Words in Transcription} \\ \hline
\multirow{2}{*}{s177} & Manual & 0\% & \textit{... OR  LIKE the cookie jar STEALING THE  cookie out of the cookie jar THE     stool **** THE TRIPLE HE  is ROCKING WITH its I WONDER IF ...}  \\ 
\hline
& TDNN & 66\% & \textit{.. HER NECK the cookie jar STANDING GROW cookie out of the cookie jar THEY'RE stool TRIP O   STOOL  SHE is WALKING IN   its * AND    THEN ...}  \\ 
\hline
\multirow{2}{*}{s192} & Manual & 0\% & \textit{... and then this here WHEN   the ***** ** IT  should be going down in there but it is going down on the side here it is going all THE way down...}  \\ 
\hline
& TDNN & 34\% & \textit{... and then this here WINDOW the WATER IN THE should be going down in there but it is going down on the side here it is going all *** way down ...}  \\ 

\bottomrule

\end{tabular}
% \vspace{-10pt}
}

\end{table*}
% \vspace{-5pt}

==> tables/keywords.tex <==



% \vspace{-10pt}
\begin{table}[htbp]
\hspace{-.35cm}
\centering
\scalebox{0.78}{
\setlength{\tabcolsep}{4pt} % column spacing
\renewcommand{\arraystretch}{1.2} % line hight

% \toprule
% \end{tabular}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\begin{tabular}{cccccc}

\toprule
\multirow{2}{*}{} & \multirow{2}{*}{WER} & \multicolumn{2}{c}{Counts} & \multicolumn{2}{c}{Errors Counts} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
 & & tokens & types & tokens & types \\
\midrule
Keywords-M & $\textbf{14.3\%}$ & $909(20\%)$ & $60(11\%)$ & $130(\textbf{9\%})$ & $46(12\%)$   \\
Non-keywords & $\textbf{35.6\%}$ & $3562(80\%)$ & $482(89\%)$ & $1270(\textbf{91\%})$ & $322(88\%)$   \\
\midrule
\midrule
Keywords-G & $\textbf{15.8\%}$ & $581(13\%)$ & $41(8\%)$ & $92(\textbf{7\%})$ & $34(9\%)$   \\
Non-keywords & $\textbf{33.6\%}$ & $3890(87\%)$ & $502(92\%)$ & $1308(\textbf{93\%})$ & $334(91\%)$   \\

\bottomrule

\end{tabular}
}
% \vspace{-0.5cm}
\caption{Word error rates (WER) and Counts (ratio \%) of manually selected keywords (Keywords-M) and GPT-generated keywords (Keywords-G) in manual transcriptions (``Trans.") and ASR errors. ``tokens" represents the count of words and ``types" represents the count of distinct words.
}
\label{tab:keywords-MS}
\vspace{-0.7cm}
\end{table}
% \vspace{-5pt}

==> tables/list_keywords.tex <==

% WER	ACC	P	R	F	A
% Manual	0	0.88	0.85	0.92	0.88	0.87
% TDNN	33.9	0.88	0.82	0.96	0.88	0.88
% Whisper	35.4	0.85	0.77	1	0.87	0.85

% \vspace{-10pt}
\begin{table}[htbp]
\vspace{-5pt}
\centering
\scalebox{0.8}{
\setlength{\tabcolsep}{4pt} % column spacing
\renewcommand{\tabularxcolumn}[1]{>{\raggedright\arraybackslash}p{#1}}
\begin{tabular}{cl}

\bottomrule

 & \makecell{Keywords} \\
\hline
\makecell{Manual} & \makecell{two, children, cookie, jar, brother, steal, cupboard, door,finger(s), \\
women, lady, dry, wash(ing), dish, water, overflow(ing), floor, \\
kitchen, window, curtain(s), mother, plate, stand, sink, boy, girl, \\
running, fall, outside, tree, house, sister, look, open, hand, glass}\\
\hline
\makecell{GPT} & \makecell{boy, reach, stool, tip, grab, stand(stood), jar, girl, look, floor,\\ worry, smile, mother(mom), wash(ing), sink, busy, turn, counter, \\
window, curtain(s), light, water, soap, cupboard, dishes, tiles}\\

\toprule

\end{tabular}
}
\caption{Manually selected and GPT-generated keywords.}
\label{tab:kwlist}
\vspace{-20pt}
\end{table}


==> tables/showcase.tex <==

% WER	ACC	P	R	F	A
% Manual	0	0.88	0.85	0.92	0.88	0.87
% TDNN	33.9	0.88	0.82	0.96	0.88	0.88
% Whisper	35.4	0.85	0.77	1	0.87	0.85

% \vspace{-10pt}
\begin{table}[htbp]
\vspace{-5pt}
\centering
\scalebox{0.9}{
\setlength{\tabcolsep}{4pt} % column spacing
\renewcommand{\tabularxcolumn}[1]{>{\raggedright\arraybackslash}p{#1}}
\begin{tabular}{lcl}

\bottomrule

Trans. & Pred. & \makecell{Trans. Text} \\
\hline
    \makecell{Manual\\(s207)} & \makecell{TN} & \makecell{
        ... \textcolor{blue}{the} boy on \textcolor{blue}{the} stool \textcolor{blue}{stool tipping} over getting \\
        \textcolor{blue}{cookie out of the} cookie jar \textcolor{blue}{mother washing \\
        dishes} water running sink overflowing ...
    }\\
\hline
    \makecell{ASR\\(s207)} & \makecell{FP} & \makecell{
        ... \textcolor{red}{a} boy on \textcolor{red}{a} stool \textcolor{red}{the winter day} over getting \\
        \textcolor{red}{***** ** ** ***} cookie jar \textcolor{red}{****** jar mhm} \\
        \textcolor{red}{****} water running \textcolor{red}{the} sink overflowing ...
    } \\
\midrule
\midrule
    \makecell{Manual\\(s177)} & \makecell{TN} & \makecell{
        ... sister I guess laughing \textcolor{blue}{at him} mother washing \\
        dishes sink is overflowing \textcolor{blue}{view of the} yard \textcolor{blue}{and} \\
        the kitchen \textcolor{blue}{window with its curtain} ...
    } \\
\hline
    \makecell{ASR\\(s177)} & \makecell{TN} & \makecell{
        ... sister I guess laughing \textcolor{red}{** ***} mother washing \\
        dishes sink is overflowing \textcolor{red}{**** ** few} yard \textcolor{red}{***} \\
        the kitchen \textcolor{red}{****** weather curtains} ...
    }\\

\toprule

\end{tabular}
}
\caption{Example transcription(``Trans.") text from participant s207 and s177, where manual and ASR transcriptions have consistent and inconsistent predictions, respectively. ``Pred.": Prediction, colored words are errors, and * is a placeholder for missing words.}
\label{tab:case}
\vspace{-20pt}
\end{table}

